Adaptive Loss Scaling for Mixed Precision Training

Mixed precision training (MPT) is becoming a practical technique to improve the speed and energy efficiency of training deep neural networks by leveraging the fast hardware support for IEEE half-precision floating point that is available in existing GPUs. MPT is typically used in combination with a technique called loss scaling, that works by scaling up the loss value up before the start of backpropagation in order to minimize the impact of numerical underflow on training. Unfortunately, existing methods make this loss scale value a hyperparameter that needs to be tuned per-model, and a single scale cannot be adapted to different layers at different training stages. We introduce a loss scaling-based training method called adaptive loss scaling that makes MPT easier and more practical to use, by removing the need to tune a model-specific loss scale hyperparameter. We achieve this by introducing layer-wise loss scale values which are automatically computed during training to deal with underflow more effectively than existing methods. We present experimental results on a variety of networks and tasks that show our approach can shorten the time to convergence and improve accuracy compared to the existing state-of-the-art MPT and single-precision floating point

==> tex/archive/intro.tex <==
\section{Introduction}

Training deep neural networks in data types with lower precision than single-precision floating-point (FP32) is gradually supported by recent hardware platforms.
For instance, IEEE half-precision floating-point (FP16), which takes 16 bits per number and uses 5 bits for exponent, 11 bits for the significand, is being supported by newly released GPU platforms \citep{nvidia-volta}.
The benefits of leveraging them are appealing: they require less memory footprint, consume less energy, and run faster compared with FP32 on the same workload.
Nevertheless, due to the relatively narrow dynamic range and low resolution of numeric values representable by them, the numerical instability of training DNN can be amplified and models cannot even be trained.

Diving into a training procedure based on SGD with decaying learning rate, we notice that problems caused by low-precision floating-point (LFP) may appear in these phases:

\begin{enumerate}[label=\textbf{(FM\arabic*)}]
    \item During the first few epochs after initialization, since the model loss is large and the learning rate is normally large, gradients are more likely to explode and step out of the dynamic range of LFP, i.e., overflow, without proper initialization.\label{fm:init}
    \item In the middle phase, some numerically unstable units, e.g., variance calculation in Batch Normalization, may produce abnormal values (NaN or Inf) and destroy training. Rounding errors introduced by LFP may also tweak the optimization direction.\label{fm:round}
    \item Around the last epochs when the learning rate is small, multiplying the learning rate by small gradients can possibly vanish to 0 due to underflow, which hinders further training.\label{fm:under}
\end{enumerate}

These three \emph{failure modes} are what we have empirically noticed while training DNN in LFP. Examples for them are shown in Figure~\ref{fig:fm}.

\begin{figure}[h]
\centering
\caption{Failure modes from training in LFP.}
\label{fig:fm}
\end{figure}

Recent literature proposes various solutions to address these failure cases.
Mixed precision training~\citep{Micikevicius2017} provides a comprehensive, state-of-the-art approach: for~\ref{fm:round}, numerically unstable units are computed in FP32 and model weights are stored in FP32 rather than LFP to avoid inaccurate accumulation by small gradient updates; loss scaling to scale up gradient updates to prevent underflow for~\ref{fm:under}.
Still, a proper solution for \ref{fm:init} is missing here and the training can still go wrong as in \figref{fig:mpt-fail}.
Also, tuning new hyperparameters from the loss scaling mechanism, as well as the necessity of supporting both FP32 and LFP are troublesome.
There are some other papers that can make further improvement.
\cite{Hoffer2018} promote the usage of $L_1$ or $L_{\infty}$ based BN for better numerical stability.
Focusing on reducing the rounding error caused by adding large and small floating-point values, i.e., swamping~\citep{Higham1993}, is an alternative approach to improve LFP training performance~\citep{Wang2018b, Sakr2019}.
\cite{Aberger2019} improve both the arithmetic precision by bit-centering and intend to address the exploding/vanishing gradient problem by reducing gradient variance through SVRG~\citep{Johnson2013}.
Floating-point itself can be improved as well, e.g., \cite{Kalamkar2019} mention the \texttt{bfloat16} that increases the ratio of the exponent to enlarge the dynamic range can empirically improve the training performance, and \cite{Johnson2018} digs into core arithmetic floating-point arithmetic for better accuracy. %TODO
In a word, almost none of these prior works provides a universal approach that addresses all the three failure modes without introducing much overhead.

\begin{figure}[h]
\centering
\caption{How mixed precision training fails when the initialization is wrong and gradient explodes.}
\label{fig:mpt-fail}
\end{figure}

Our paper aims to resolve all these failure modes in an efficient manner.
We stick to FP16 due to its universality on recent hardware platforms, and we prefer a hyperparameter-free and FP32-free approach to reduce the overhead for usage.
% 
For \ref{fm:init}, we first dive into the initialization problem to ensure that at least in the first few epochs, gradients and activations will stay in the dynamic range.
We extend the \emph{fixup} initialization method~\citep{Zhang2019}, which produces the state-of-the-art performance on over 10k layers DNN, to take into account the dynamic range of FP16.
%
The numerical instability mentioned in~\ref{fm:round} caused by BN can be addressed by fixup in the sense that they replace BN by a trainable affine transformation.
Surprisingly, those rounding errors that are deliberately addressed by some prior works, are not significantly harmful to the validation accuracy based on our empirical study, especially when the model is overparameterized.
%
Regarding the vanishing gradient problem incurred by underflow as in~\ref{fm:under}, instead of treating the small learning rate as it is, we choose to improve the learning rate schedule such that the total amount of underflow will be constrained by a threshold.
%
Moreover, our method is parameterised regarding the floating-point configuration, the number of exponent and significand bits $(N_E, N_S)$ is populated to the solutions we give. 

To be specific, our method is a combination of applying the following solutions:

\begin{enumerate}[label=\textbf{(FS\arabic*)}, itemsep=0em]
    \item Improve the fixup initializer to take into account the dynamic range of FP16 and avoid exploding gradient.
    \item Empirically study the effect of removing BN and using BN alternatives, as well as the rounding errors. % TODO
    \item Change the learning rate schedule of SGD-based and adaptive optimizers to reduce the amount of underflow gradient updates.
\end{enumerate}

Our method can achieve ...

==> tex/archive/main.tex <==
\input{tex/intro.tex}
\input{tex/method.tex}



==> tex/archive/method.tex <==
\input{tex/method/initialization.tex}
\input{tex/method/rounding_error.tex}
\input{tex/method/optimizer.tex}


==> tex/archive/method/initialization.tex <==
\section{Initialization}

==> tex/archive/method/optimizer.tex <==
\section{Optimization}

==> tex/archive/method/rounding_error.tex <==
\section{Rounding Error}

==> tex/experiment/ablation.tex <==
\subsection{Ablation Study}\label{sec:exp:ablation}

% Why adaptive loss scaling is better than a fixed one, down to the lowest level
% Show the comparison of zeroed out gradients in different cases
% Would different layers use different scale?

% Is the assumption of data distribution correct?

==> tex/experiment/deep_mlp.tex <==
\subsection{Deep MLP}

Deep MLP is frequently used to study the exploding and vanishing gradient problem in training deep learning models.
Therefore, testing different loss scaling methods under the mixed precision framework for deep MLP helps us measure the effectiveness of adaptive loss scaling for addressing such problems.
We train MLP with the same number of hidden units per layer, but different depth, with various loss scaling methods on the MNIST dataset.
Each layer in this MLP is followed by ReLU only, without batch normalization.
Each MLP instance is trained by the same schedule for all loss scaling methods, specifically, taking 10 epochs and using $1e^{-3}$ learning rate.
Weights among all layers are initialized through the approach in~\citep{He2015a}.

% show the plot here

==> tex/method/adaptive.tex <==
\subsection{Problem Formulation}

Here we consider a multi-layer perceptron (MLP) model that consists of matrix multiplication.
Suppose $\mX_i$ is the input to layer $i$, $\mW_i$ indicates its weights, the output $\mX_{i+1}$ equals to $\mW_i \mX_i$.
Given the empirical loss as $\mathcal{L}$, the gradient backpropagated to layer $i$ as $\nicefrac{\partial\mathcal{L}}{\partial\mX_{i+1}}$, and ,
The gradient backpropagated to $\mX_i$ is scaled by $\prod_{j=i+1}^{L+1} \alpha_{j}$, i.e., $\prod_{j=i+1}^{L+1} \alpha_{j} \partial \mathcal{L}/\partial \mY_i$.
In total there are $L$ sequentially connected layers, and our objective is that, given an initial $\alpha_{L+1}$, we need to decide all the $\alpha_i$, $1 \leq i \leq L$ such that the amount of elements in activation gradients $\partial \mathcal{L}/\partial \mY_i$ is largely reduced.

\begin{equation}
    \begin{aligned}
    \alpha_i^t = \argmin_{\alpha}\ 
        \mathcal{C}
        \left(
            \alpha
            \left( \prod_{j=i+1}^{L+1} \alpha_{j}^t \right)
            \Delta \mX_{i+1}^t
            \mW_i^{t-1}
        \right)
    \end{aligned}
\end{equation}

We assume that the product $p$ between an input gradient and a weight is drawn from a normal distribution $\normal(\mu_p, \sigma_p^2)$~\citep{He2015a}, weights are generated i.i.d from a distribution with mean and variance $\sigma_w^2$, and elements in $\Delta \mX_{i+1}^t$ are also i.i.d from a distribution with mean $\mu_g$ and variance $\sigma_g^w$.
We can further deduce $\mu_p$ and $\sigma_p^2$ by~\eqref{eq:pprob}.

\begin{equation}\label{eq:pprob}
   \mu_p = \mu_w \mu_g\quad
   \sigma_p^2 = (\sigma_w^2 + \mu_w^2) (\sigma_g^2 + \mu_g^2) - \mu_g^2 \times \mu_w^2
\end{equation}

Furthermore, we assume $\mu_w$ to be 0. $p$ then has zero mean, and the absolute value of $p$ forms a half-normal distribution.
We intend to constrain the amount of $|p|$ values that are below the minimal denormal number of FP16 $u_{\min}$, denoted by $N_{uf}$, within a threshold $t$.
We can derive $N_{uf}$ by the CDF of $|p|$, which is $\mathrm{erf}(\nicefrac{u_{\min}}{\sqrt{2}\sigma_p})$.
If we scale the input gradient by $\alpha$ in order to constrain $N_{uf}$ under $t$, we can deduce the minimal value of $\alpha$ that can be taken:

\begin{equation}
   t \geq P(\alpha \times |p| \leq u_{\min}) = \mathrm{erf}(\frac{u_{\min}}{\sqrt{2}\alpha\sigma_p}) 
   \Longleftrightarrow
   \alpha \geq \frac{u_{\min}}{\mathrm{erf}^{-1}(t) \sqrt{2} \sigma_p}
\end{equation}

\begin{equation}
    p = g \times w
\end{equation}

\begin{equation}
    p \sim \normal(0, \sigma_p^2)
\end{equation}


==> tex/method/impl.tex <==
% NOTE: we may put this section in the supplementary part
\subsubsection{Post-processing}\label{sec:impl}

A raw loss scale value calculated from \Eqref{eq:loss_scale:gemm} should be post-processed by the following rules:

\begin{enumerate}
\item
Most importantly, it should be rounded down to the nearest \textbf{power-of-two} number.
Otherwise, due to the nature of floating-point, a scaled gradient cannot always be unscaled by the same scale, i.e., $(\alpha x)/\alpha \neq x$ if $\alpha$ is not a power of two~\citep{Muller}.

\item
Besides this rule, we also give an upper bound of the total accumulated loss scale value to prevent it going too large and amplifying low-precision arithmetic errors, although it is pretty rare based on our empirical evaluation and we fix this bound to 2048 as a constant.

\item
The upper bound of loss scale is determined by avoiding overflow.
For the GEMM case, it can be simply calculated by choosing the maximal numbers from both operands, multiplying them together, and then taking 1 over that multiplication result as the largest possible loss scale, i.e., $1/(\max(\mW) \times \max(\vdelta))$.
This is a loose bound since these selected maximal numbers may not be multiplied together when calculating the output activation gradient.
In practice, this upper bound is much larger than the lower bound, and we simply choose the lower bound as the loss scale value, and only switch to the upper bound only when the upper bound is smaller than the lower bound.
Other operators will not update loss scale (except branching, which has been discussed in \Secref{sec:loss_scale_calc:elemwise}), we assume they will not cause overflow.
\end{enumerate}



==> tex/method/loss_scaled_backprop/backprop.tex <==
% \subsubsection{Backpropagation Algorithm}

\begin{algorithm}
    \DontPrintSemicolon
    \caption{Backpropagation algorithm with adaptive loss scaling.
    Assuming each layer has a single output.}
    \label{alg:backprop}

    \SetKwFunction{FGetLayerOutput}{GetLayerOutput}
    \SetKwFunction{FGetLossScale}{GetLossScale}
    \SetKwFunction{FBackprop}{Backprop}
    \SetKwFunction{FOp}{OP}

    $\sgrad{\alpha_{N+1}}{\vdelta_{N+1}} \gets $ initial loss scale, and error gradient \emph{scaled} by $\alpha_0$\;
    \For{$i \gets $ layer ID in a reversed topological order}{
        $j$         $\gets$ \FGetLayerOutput{$i$}\;
        $\beta_i$   $\gets$ \FGetLossScale{\FOp{$i$}, $\sgrad{\alpha_j}{\vdelta_j}$}\;
        $\vdelta_i$ $\gets$ \FBackprop{\FOp{$i$}, $\beta_i\vdelta_j$}\;
        $\alpha_i$  $\gets$ $\alpha_j\beta_i$\;
    }
\end{algorithm}

In general, the adaptive loss scaled backpropagation works as shown in the pseudocode of \Algref{alg:backprop}.
At the beginning, we have an initial error gradient, directly calculated from the loss value and the final output.
We may optionally scale this gradient by a manually set value $\alpha_{N+1}$.
Next, we traverse the computation graph of the neural network in a reversed topological order, i.e., move to a new layer until all its output layers have been visited.
This stays the same as the canonical way of backpropagation.
We cover single-output cases for simplicity at this stage, and we will dive into detail about how to handle branch output in the following sections.
When visiting each layer $i$, we retrieve the tuple $\sgrad{\alpha_j}{\vdelta_j}$ propagated to it from output layers and calculate a local loss scale value $\beta_i$.
This local value will be multiplied to $\vdelta_j$ \emph{before} we calculate the gradient for previous layers, as well as the gradient update for weights of layer $i$ (omitted in the algorithm).
Since $\beta_i$ contributes to the magnitude of the gradient $\vdelta_i$, we can calculate the loss scale value corresponds to $\vdelta_i$ by $\alpha_j\beta_i$.
Looking back to the $N$-layer MLP example, from this algorithm, we can realize that the loss scale value from layer $i$ is an accumulation of $\beta_i$ all its following layers' scales, i.e., $\alpha_i=\alpha_{N+1}\prod_{j=i}^{N} \beta_j$.



==> tex/method/loss_scaled_backprop/loss_scaled_grad.tex <==
% \subsubsection{Loss Scaled Gradient}
% \label{sec:method:loss_scaled_backprop:loss_scaled_grad}

% During a standard backpropagation process, only gradients are passed through every layer.
% If the gradient has been scaled by a loss scale before backpropagation happens, each layer still takes in and produces gradients as the normal backpropagation procedure, and the only difference is that all layers can access to a global loss scale value $\alpha$, which will be used to unscale gradient for weight update.
% In the case of adaptive loss scaling, since we assign a distinct loss scale value per layer, \emph{both gradients and their corresponding loss scale values should be propagated}.
